OpenWAM: An Open Framework for Composable World-Action Models

World-action models (WAMs) couple future prediction with robot control, yet existing systems often vary the video backbone, interaction structure, supervision, and inference procedure simultaneously, making their design choices difficult to compare. We introduce OPENWAM, an open world-action modeling framework built around a common causal robot-video foundation and configurable video-action interaction. Starting from Wan2.2-5B, we perform causal robot-video pretraining on over 10,000 hours of video, then integrate an action expert through a shared Mixture-of-Transformers architecture that supports joint, video-then-action, action-then-video, and decoupled generation. OPENWAM achieves high success rates on four LIBERO suites and real-world bimanual tasks; robot-video training with causal adaptation improves VTA success on LIBERO-Long from 68.4% to 97.8%. The same configurable architecture naturally extends to inverse and forward dynamics, allowing us to study how counterfactual transitions improve independently trained dynamics models beyond demonstrations alone. When only the video predictor is adapted to a new task, a frozen local-context inverse dynamics model trained on counterfactual data and demonstrations achieves 84.0% mean success across four held-out LIBERO-90 tasks, compared with 47.0% for a full-context inverse model and 21.5% for a local-context model trained only on demonstrations. For forward dynamics, counterfactual supervision reduces RGB prediction error by 34.5% and raises outcome identification from 21.1% to 71.3% among 16 same-state outcomes. OPENWAM provides a common testbed for comparing WAM interaction designs and for studying dynamics learning from video data beyond successful demonstrations.

==> sec/tables/main_results_v2.tex <==
\begin{table*}[t]
\centering
\small
\setlength{\tabcolsep}{4pt}

% ------------ Left table: QuantiPhy evaluation ------------
\begin{minipage}[t]{0.61\textwidth}
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{
r|
>{\centering\arraybackslash}p{1.2cm}|
>{\centering\arraybackslash}p{1.2cm}
>{\centering\arraybackslash}p{1.2cm}
>{\centering\arraybackslash}p{1.2cm}
>{\centering\arraybackslash}p{1.2cm}|
>{\centering\arraybackslash}p{1.2cm}
}
\toprule
\multicolumn{1}{c}{\multirow{2}{*}{Models}}  & \multicolumn{1}{c}{\multirow{2}{*}{Size}}   &
\multicolumn{4}{|c|}{\textbf{Kinematic Categories}} & \multicolumn{1}{c}{\multirow{2}{*}{Avg.}} \\
 \multicolumn{1}{c}{}&  \multicolumn{1}{c}{} &  \multicolumn{1}{|c}{2S}  & \multicolumn{1}{c}{2D}  & \multicolumn{1}{c}{3S}  & \multicolumn{1}{c|}{3D} &  \\
\midrule
\rowcolor{row_color}
\multicolumn{7}{l}{\textit{Proprietary models}} \\
\includegraphics[height=0.75em]{sec/images/icons/medal1.png}\ ChatGPT-5.1~\cite{OpenAIgpt5.1} & -- & \bestsub{46.3} & 56.2 & \bestsub{51.5} & \bestsub{58.3} & \best{53.1} \\
\includegraphics[height=0.75em]{sec/images/icons/medal2.png}\ Gemini-2.5 Pro~\cite{google2025gemini25pro} & -- & 44.8 & \bestsub{57.5} & 42.4 & 53.7 & 49.6 \\
\includegraphics[height=0.75em]{sec/images/icons/medal3.png}\ Gemini-2.5 Flash~\cite{google2025gemini25flash} & -- & 40.3 & 53.2 & 43.6 & 57.4 & 48.6 \\
Grok 4.1 (Fast Reasoning)~\cite{grok41} & -- & 39.4 & 49.5 & 42.4 & 48.6 & 45.0 \\
ChatGPT-5~\cite{OpenAIgpt5} & -- & 36.6 & 35.0 & 25.9 & 33.1 & 32.6 \\
Claude Sonnet 4.5~\cite{anthropic2025claude45sonnet} & -- & 19.6 & 23.0 & 19.6 & 29.1 & 22.8 \\
\midrule
\rowcolor{row_color}
\multicolumn{7}{l}{\textit{Open-weight models}} \\
\includegraphics[height=0.75em]{sec/images/icons/medal1.png}\ Qwen3-VL-Instruct-32B~\cite{bai2025qwen25vl} & 32B & 35.8 & \bestopensub{51.6} & \bestopensub{43.2} & \bestopensub{53.4} & \bestopen{46.0} \\
\includegraphics[height=0.75em]{sec/images/icons/medal2.png}\ InternVL-3.5-30B~\cite{chen2024internvl} & 30B & \bestopensub{36.7} & 45.4 & 38.6 & 42.0 & 40.7 \\
\includegraphics[height=0.75em]{sec/images/icons/medal3.png}\ Qwen3-VL-Instruct-8B~\cite{bai2025qwen25vl} & 8B & 26.0 & 47.8 & 35.1 & 46.3 & 38.8 \\
InternVL-3.5-8B~\cite{chen2024internvl} & 8B & 27.3 & 41.8 & 34.4 & 38.3 & 35.4 \\
Molmo-7B~\cite{allenai2025molmo} & 7B & 30.0 & 43.1 & 24.4 & 36.6 & 33.5 \\
Phi-4-Multimodal-Instruct~\cite{microsoft2025phi4multi} & 5.6B & 33.4 & 42.3 & 25.4 & 28.4 & 32.4 \\
Qwen3-VL-Instruct-2B~\cite{bai2025qwen25vl} & 2B & 27.1 & 39.0 & 17.6 & 32.1 & 29.0 \\
SmolVLM-Instruct~\cite{marafioti2025smolvlm} & 0.26B & 31.6 & 34.4 & 20.0 & 27.8 & 28.5 \\
InternVL-3.5-2B~\cite{chen2024internvl} & 2B & 25.0 & 31.1 & 16.6 & 27.4 & 25.0 \\
VILA-7B~\cite{lin2023vila} & 7B & 23.0 & 29.8 & 14.4 & 23.0 & 22.6 \\
CogVLM2 Video~\cite{wang2024cogvlm2} & 12B & 19.4 & 28.7 & 12.7 & 27.9 & 22.2 \\
Phi-3-Mini-128K-Instruct-3.8B~\cite{microsoft2024phi3} & 3.8B & 17.3 & 14.7 & 19.5 & 18.6 & 17.5 \\
LLaVA-13B~\cite{liu2023visual} & 13B & 14.4 & 22.1 & 8.0 & 16.5 & 15.2 \\
MiniCPM-V 4.5~\cite{yao2024minicpmv} & 8B & 27.6 & 26.3 & 0.4 & 0.0 & 13.6 \\
Fuyu-8B~\cite{adept2023fuyu} & 8B & 9.5 & 14.7 & 9.5 & 16.2 & 12.5 \\
\midrule
\textcolor{gray}{Human Baseline} & \textcolor{gray}{--} &
\textcolor{gray}{50.0} & \textcolor{gray}{59.1} &
\textcolor{gray}{55.2} & \textcolor{gray}{57.9} & \textcolor{gray}{55.6} \\
\bottomrule
\end{tabular}
}
\caption{
Evaluation results on \textsc{QuantiPhy}. We report Mean Relative Accuracy (MRA \%) on four kinematic categories (2S, 2D, 3S, 3D) and their average. \best{Dark} cell marks the best overall model and \bestopen{light} cell marks the best open-weight model.
}
\label{tab:main-results}
\end{minipage}
\hfill
% ------------ Right table: Ablations (no model or size column) ------------
\begin{minipage}[t]{0.35\textwidth}
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{
>{\centering\arraybackslash}p{1.7cm}|
>{\centering\arraybackslash}p{1.7cm}|
>{\centering\arraybackslash}p{1.9cm}|
>{\centering\arraybackslash}p{1.4cm}
}
\toprule
\multicolumn{1}{c}{\multirow{2}{*}{Video + Prior}} &
\multicolumn{1}{c}{\multirow{2}{*}{Prior only}} &
\multicolumn{1}{c}{\multirow{2}{*}{Counterfactual}} &
\multicolumn{1}{c}{\multirow{2}{*}{CoT}} \\
\multicolumn{1}{c}{} &
\multicolumn{1}{c}{} &
\multicolumn{1}{c}{} &
\multicolumn{1}{c}{} \\
\midrule
\rowcolor{row_color}
\multicolumn{4}{l}{\textit{}} \\

56.1 & 39.0 & 15.4 & 27.7 \\ % gpt-5.1
60.9 & 46.1 & 29.9 & 49.8 \\ % gemini-2.5-pro
49.8 & 36.1 & 14.4 & 22.4 \\ % gemini-flash
47.5 & 44.3 & 31.6 & 39.5 \\ % grok
34.2 & 50.8 & 29.6 & 53.7 \\ % gpt-5
25.4 & 16.6 & 11.6 & 25.9 \\ % claude

\midrule
\rowcolor{row_color}
\multicolumn{4}{l}{\textit{}} \\

50.1 & 37.2 & 34.0 & 23.1 \\ % Qwen3-32B
45.4 & --   & 12.1 & 17.6 \\ % InternVL-30B
40.5 & 24.9 & 12.0 & 21.0 \\ % Qwen3-8B 
37.0 & 19.3 & 29.7 & 18.2 \\ % InternVL-8B 
39.8 & --   & 14.7 & 15.9 \\ % molmo 
40.0 & 20.1 & 9.2  & 23.5 \\ % Phi-4 
34.9 & 28.2 & 25.2 & 25.6 \\ % Qwen3-2B
38.9 & --   & 14.3 & 17.8 \\ % smolvlm
32.7 & 25.1 & 22.5 & 21.5 \\ % InternVL-2B 
31.8 & --   & 14.1 & 10.0 \\ % vila
28.5 & --   & 9.5  & 26.4 \\ % cogvlm2
11.1 & 10.3 & 8.4  & 7.2  \\ % phi-3 
20.2 & --   & 13.9 & 14.4 \\ % llava 
29.7 & --   & 19.9 & 24.1 \\ % minicpm 
14.3 & --   & 9.0  & 21.1 \\ % fuyu

\midrule
\textcolor{gray}{--} & \textcolor{gray}{--} &
\textcolor{gray}{--} & \textcolor{gray}{--} \\
\bottomrule
\end{tabular}
}
\caption{Extensive results on an analysis subset. We report Mean Relative Accuracy (MRA) in \%. Rows follow the same model order as in Table~\ref{tab:main-results}.} 


\label{tab:more-results}
\end{minipage}

\end{table*}


==> sec/tables/tab_parsing-examples1.tex <==
\begin{tabular}{@{} c L{7.5cm} L{4.0cm} L{3.0cm} @{}}
\toprule
\textbf{\#} & \textbf{Question} & \textbf{GT Prior} & \textbf{GT Depth Info} \\
\midrule
1 & What is the length of the slope in cm? & $t=0.6$, ball acc. $= 4.6\text{m/s}^2$ & $t=0\text{s}$, dist. $\text{slope\_far} = 1.8540\text{m}$, dist. $\text{slope\_near} = 1.7010\text{m}$ \\
2 & What is the basketball's distance from the camera at $1.2\text{s}$ in meters? & acc. $= 9.8 \text{m/s}^2$ & $t=1.0\text{s}$, dist. $\text{ball} = 1.4010\text{m}$, $t=1.2\text{s}$, dist. $\text{ball} = 1.5640\text{m}$ \\
3 & What is the basketball's distance from the camera at $1.2\text{s}$ in meters? & acc. $= 9.8 \text{m/s}^2$ & $t=1.0\text{s}$, dist. $\text{ball} = 1.4010\text{m}$, $t=1.2\text{s}$, dist. $\text{ball} = 1.5640\text{m}$ \\
4 & What is the velocity of the ball at the end of the slope in cm/s? & $t=1.4$, ball acc. $= 4.05\text{m/s}^2$ & $t=1.0\text{s}$, dist. $\text{ball} = 1.7790\text{m}$, dist. $\text{slope\_far\_end} = 1.8150\text{m}$ \\
5 & What is the velocity of the soccer ball at $1.5\text{s}$ in m/s? & gravity acc. $= 9.8\text{m/s}^2$ & $t=1.5\text{s}$, dist. $\text{soccer\_ball} = 1.4020\text{m}$ \\
6 & What is the velocity of the tennis ball at $3.4\text{s}$? & gravity acc. $= 9.8\text{m/s}^2$ & dist. $\text{near\_person} = 2.002\text{m}$, dist. $\text{far\_person} = 3.130\text{m}$ \\
7 & What is the acceleration of the red ball at $0.2\text{s}$ in $\text{cm/s}^2$? & diameter of the red ball $= 7\text{cm}$ & $t=0.2\text{s}$, dist. $\text{book} = 1.0995\text{m}$, $t=0.6\text{s}$, dist. $\text{book} = 1.1510\text{m}$ \\
8 & What is the shoulder breadth of the person in cm? & gravity acc. $= 9.8\text{m/s}^2$ & \\
9 & What is the basketball's diameter in cm? & acc. $= 9.8 \text{m/s}^2$ & $t=1.0\text{s}$, dist. $\text{ball} = 1.4010\text{m}$, $t=1.2\text{s}$, dist. $\text{ball} = 1.5640\text{m}$ \\
10 & What is the velocity of the toy at $2.6\text{s}$ in $\text{cm/s}$? & gravity acc. $= 9.8\text{m/s}^2$ & \\
11 & What is the velocity of the toy at $2.6\text{s}$ in $\text{cm/s}$? & gravity acc. $= 9.8\text{m/s}^2$ & \\
12 & What is the diameter of the tennis ball in cm? & gravity acc. $= 9.8\text{m/s}^2$ & dist. $\text{near\_person} = 2.002\text{m}$, dist. $\text{far\_person} = 3.130\text{m}$ \\
13 & What is the length of the wood block in cm? & ruler calibre $= 1\text{cm}$ & \\
14 & What is the acceleration of the astronaut at time $1\text{s}$ in $\text{m/s}^2$? & height of the astronaut $= 2.2\text{m}$ & $t=1\text{s}$, dist. $\text{astronaut} = 23.137\text{m}$ \\
15 & What is the acceleration of the tennis ball at time $1.5\text{s}$ in $\text{m/s}^2$? & diameter of the tennis ball $= 0.17\text{m}$ & \\
16 & What is the diameter(width) of the plant in meters? & acc. of the mug cup before $0.5\text{s} = 9.8\text{m/s}^2$ & \\
17 & What is the velocity of the ball at the end of the slope in cm/s? & $t=1.4$, ball acc. $= 4.05\text{m/s}^2$ & $t=1.0\text{s}$, dist. $\text{ball} = 1.7790\text{m}$, dist. $\text{slope\_far\_end} = 1.8150\text{m}$ \\
18 & What is the diameter of the soccer ball in cm? & gravity acc. $= 9.8\text{m/s}^2$ & dist. $\text{near\_person} = 2.002\text{m}$, dist. $\text{far\_person} = 3.130\text{m}$ \\
19 & What is the distance between two people in cm? & gravity acc. $= 9.8\text{m/s}^2$ & $t=0.60\text{s}$, dist. $\text{near\_person} = 1.5800\text{m}$, dist. $\text{far\_person} = 3.2370\text{m}$ \\
20 & What is the height of the person in cm? & gravity acc. $= 9.8\text{m/s}^2$ & \\
21 & What is the height of the toy in cm? & gravity acc. $= 9.8\text{m/s}^2$ & \\
22 & What is the width of the box in cm? & gravity acc. $= 9.8\text{m/s}^2$ & dist. $\text{near\_person} = 2.002\text{m}$, dist. $\text{far\_person} = 3.130\text{m}$ \\
23 & What is the height of the yellow toy in cm? & gravity acc. $= 9.8\text{m/s}^2$ & $t=0.60\text{s}$, dist. $\text{jar} = 1.9735\text{m}$, dist. $\text{carrot} = 2.6300\text{m}$ \\
24 & What is the basketball's diameter in cm? & acc. $= 9.8 \text{m/s}^2$ & $t=1.0\text{s}$, dist. $\text{ball} = 1.4010\text{m}$, $t=1.2\text{s}$, dist. $\text{ball} = 1.5640\text{m}$ \\
25 & What is the height of the woman in yellow in meters? & walking velocity $= 1.25\text{m/s}$ & \\
26 & What is the length of the speedboat in meters? & sailboat length $= 12\text{m}$ & \\
27 & What is the length of the string in cm? & gravity acc. $= 9.8 \text{m/s}^2$ & $t=0.3\text{s}$, dist. $\text{ball} = 1.7060\text{m}$, $t=0.6\text{s}$, dist. $\text{ball} = 1.3440\text{m}$ \\
28 & What is the displacement of the rolling object from $0\text{s}$ to $0.6\text{s}$ in cm? & $t=0.6$, ball acc. $= 4.6\text{m/s}^2$ & $t=0\text{s}$, dist. $\text{ball} = 1.8180\text{m}$, $t=0.6\text{s}$, dist. $\text{ball} = 1.7288\text{m}$ \\
29 & What is the basketball's distance from the camera at $1.8\text{s}$ in meters? & acc. $= 9.8 \text{m/s}^2$ & $t=0.0\text{s}$, dist. $\text{ball} = 1.3210\text{m}$, $t=1.8\text{s}$, dist. $\text{ball} = 1.5835\text{m}$ \\
30 & What is the velocity of the tennis ball at $3.4\text{s}$? & gravity acc. $= 9.8\text{m/s}^2$ & dist. $\text{near\_person} = 2.002\text{m}$, dist. $\text{far\_person} = 3.130\text{m}$ \\
31 & What is that ball's acceleration at $0.6\text{s}$ in m/s? & gravity acc. $= 9.8 \text{m/s}^2$ & $t=0.3\text{s}$, dist. $\text{ball} = 1.7060\text{m}$, $t=0.6\text{s}$, dist. $\text{ball} = 1.3440\text{m}$ \\
32 & What is the width of the desk in cm? & $t=1.5$, ball acc. $= 3.0\text{m/s}^2$ & $t=0\text{s}$, dist. $\text{cup} = 1.2100\text{m}$, dist. $\text{desk\_left} = 0.8690\text{m}$ \\
33 & What is the length of the slope in cm? & $t=1.5$, ball acc. $= 3.0\text{m/s}^2$ & $t=0\text{s}$, dist. $\text{slope\_far} = 1.3450\text{m}$, dist. $\text{slope\_near} = 1.1040\text{m}$ \\
34 & What is the length of the box in cm? & gravity acc. $= 9.8\text{m/s}^2$ & dist. $\text{near\_person} = 2.002\text{m}$, dist. $\text{far\_person} = 3.130\text{m}$ \\
\bottomrule
\end{tabular}


==> sec/tables/tab_parsing-examples2.tex <==
\begin{tabular}{@{} c c c C{2.0cm} L{5.0cm} C{1.4cm} L{3.2cm} @{}}
\toprule
\textbf{\#} & \textbf{Video Type} & \textbf{Inference Type} & \textbf{GT Posterior} & \textbf{Raw Response} & \textbf{Parsed Value} & \textbf{Model} \\
\midrule
1 & A3MS & DS & 30.8 & Looking at the video frames, I can see a table $\dots$ Length $= 0.1530\text{m} = 15.30\text{cm}$ & 15.30 & Claude-4.5 Sonnet \\
2 & A3SS & DS & 1.565 & $1.5640 \text{m}$ & 1.564 & Claude-4.5 Sonnet \\
3 & A3SS & DS & 1.565 & $[1.5640]$ & 1.564 & CogVLM2 Video \\
4 & A3SS & DD & 208.76 & $[\text{velocity\_at\_the\_end\_of\_the\_slope}]$ $[\text{unit}]$ & None & CogVLM2 Video \\
5 & A3SS & DD & 2.7968 & $1.5 \text{m/s}$ \textbackslash n In the given video, the soccer ball is flying $\dots$ at 1.5 m/s. & 1.5 & Fuyu-8B \\
6 & A3MC & DD & 542.82 & $2.002\text{m/s}$ \textbackslash n In the image, $\dots$ Therefore, its velocity is 2.002m/s. & 2.002 & Fuyu-8B \\
7 & S3SC & SD & 1086.09 & $0.0 \text{cm/s}^2$ & 0 & Gemini-2.5 Flash \\
8 & A2MC & DS & 39 & $39.8 \text{cm}$ & 39.8 & Gemini-2.5 Flash \\
9 & A3SS & DS & 23.2 & $23.9 \text{cm}$ & 23.9 & Gemini-2.5 Pro \\
10 & A2MS & DD & 357 & $0 \text{cm/s}$ & 0 & Gemini-2.5 Pro \\
11 & A2MX & DD & 357 & $-2549 \text{cm/s}$ & 2549 & ChatGPT-5.1 \\
12 & A3MC & DS & 6.7 & $6.5 \text{cm}$ & 6.5 & ChatGPT-5.1 \\
13 & S2MC & SS & 9.9 & $10 \text{cm}$ & 10 & ChatGPT-5 \\
14 & S3SS & SD & 3.604 & $0 \text{m/s}^2$ & 0 & ChatGPT-5 \\
15 & S2SS & SD & 6.129 & $9.8 \text{m/s}^2$ & 9.8 & InternVL-3.5-30B \\
16 & A2MC & DS & 0.075 & $0.05 \text{m}$ & 0.05 & InternVL-3.5-30B \\
17 & A3SS & DD & 208.76 & $[4.05]$ $[\text{m/s}^2]$ & 4.05 & LLaVA-13B \\
18 & A3MX & DS & 17.5 & $[0.31]$ $[0.28]$ & 0.28 & LLaVA-13B \\
19 & A3MX & DS & 325 & $[3.2370]$ $[\text{m}]$ & 3.237 & LLaVA-13B \\
20 & A2MC & DS & 170 & <think>
So, let's try to $\dots$ maybe the person's height is around $170 \text{cm}$. & 170 & MiniCPM-V 4.5-8B \\
21 & A2MX & DS & 14 & $<\text{think}>$ Okay, so I need to $\dots$ If I can determine the time it & None & MiniCPM-V 4.5-8B \\
22 & A3MX & DS & 7.2 & $0.000000000000000000000\dots$ & 0 & Molmo-7B \\
23 & A3MS & DS & 14 & $15.2 \text{cm}$ & 15.2 & Molmo-7B \\
24 & A3SS & DS & 23.2 & $23.9 \text{cm}<|\text{end}|>$ & 23.9 & Phi-3-Mini-128K-Instruct \\
25 & V2MC & DS & 1.71 & Cannot be determined from given information. & None & Phi-3-Mini-128K-Instruct \\
26 & S2MC & SS & 4.8 & $[\text{Value missing due to insufficient information}]$ & None & Phi-3-Mini-128K-Instruct \\
27 & A3SS & DS & 30 & $34.02 \text{cm}$ & 34.02 & Phi-4-Multimodal-Instruct \\
28 & A3MC & DS & 207.9 & $-22.8 \text{cm}$ & 22.8 & Phi-4-Multimodal-Instruct \\
29 & A3SC & DS & 1.5835 & $1.5835 \text{m}$ & 1.5835 & Qwen3-VL-Instruct-8B \\
30 & A3MC & DD & 542.82 & $0.0 \text{m/s}$ & 0 & Qwen3-VL-Instruct-8B \\
31 & A3SS & DS & 4.939 & $0.000000000000000000000\dots$ & 0 & VILA-7B \\
32 & A3MX & DS & 857.9 & $1.2100 \text{m}$ & 1.21 & VILA-7B \\
33 & A3MS & DS & 30.8 & $13450$ & 13450 & SmolVLM-Instruct \\
34 & A3MC & DS & 19.5 & $1.50000000000000004$ & 1.5 & SmolVLM-Instruct \\
\bottomrule
\end{tabular}
